Argument Generation with Retrieval, Planning, and Realization

Automatic argument generation is an appealing but challenging task. In this paper, we study the specific problem of counter-argument generation, and present a novel framework, CANDELA. It consists of a powerful retrieval system and a novel two-step generation model, where a text planning decoder first decides on the main talking points and a proper language style for each sentence, then a content realization decoder reflects the decisions and constructs an informative paragraph-level argument. Furthermore, our generation model is empowered by a retrieval system indexed with 12 million articles collected from Wikipedia and popular English news media, which provides access to high-quality content with diversity. Automatic evaluation on a large-scale dataset collected from Reddit shows that our model yields significantly higher BLEU, ROUGE, and METEOR scores than the state-of-the-art and non-trivial comparisons. Human evaluation further indicates that our system arguments are more appropriate for refutation and richer in content.

==> motivating_examples.tex <==
CMV: Gun control will do nothing to solve gun violence. 

ours-6-new: there are a number of reasons why gun control is a good idea . there are plenty of guns in the united states that have a large number of gun owners . if you look at the number of people in the us , there are very few guns in the world that are going to be banned in the first place . there are a lot of people who are in favor of gun control , but there are still plenty of people who do n't want to ban guns . it 's not like guns are banned because they are n't banned .

passage-1: dershowitz is a strong supporter of gun control . he has criticized the second amendment to the united states constitution , saying that it has " no place in modern society " . dershowitz supports repealing the amendment , but he vigorously opposes using the judicial system to read it out of the constitution because it would open the way for further revisions to the bill of rights and constitution by the courts . " foolish liberals who are trying to read the second amendment out of the constitution by claiming it 's not an individual right or that it 's too much of a public safety hazard do n't see the danger in the big picture.dershowitz supports repealing the amendment , but he vigorously opposes using the judicial system to read it out of the constitution because it would open the way for further revisions to the bill of rights and constitution by the courts . " foolish liberals who are trying to read the second amendment out of the constitution by claiming it 's not an individual right or that it 's too much of a public safety hazard do n't see the danger in the big picture . they 're courting disaster by encouraging others to use the same means to eliminate portions of the constitution they do n't like . "


passage-2: assessing gun control published : october 3 , 2003 atlanta , oct. 2 — a review of gun control laws , including mandatory waiting periods and bans on certain weapons , found no proof that they reduce firearm violence , the centers for disease control and prevention said on thursday . the agency said the report suggested more study was needed , not that the laws had failed . but critics said the report might be used to undercut the gun control movement . a task force of scientists appointed by the agency reviewed 51 studies about the effectiveness of eight types of gun control laws . the laws included bans on specific firearms or ammunition , prohibitions against felons buying guns , and mandatory waiting periods and firearm registration.but critics said the report might be used to undercut the gun control movement . a task force of scientists appointed by the agency reviewed 51 studies about the effectiveness of eight types of gun control laws . the laws included bans on specific firearms or ammunition , prohibitions against felons buying guns , and mandatory waiting periods and firearm registration . none of the studies were done by the federal government . in every case , the task force found '' insufficient evidence to determine effectiveness . ''


passage-3: 	the solution has to be elsewhere in reducing drugs , street gangs , longer jail terms , community involvement , more police , reduction of violence in entertainment , responsible parenting , increase of hope for the downtrodden with better education and economic expansion . the solution , if there is one , is very complex and difficult . the problems are not caused by the nra , but is function of our violent society . guns will be available to those with criminal intent and most of these weapons are already illegal . the majority of guns used in these terrible street shootings are already “ outlawed ” and are not legal . so i can only assume “ bfstk ” that you want to make illegal , illegal firearms .

--------------------------------------------------------------------
CMV: Journalism has become so biased in this country that it has lost its relevance.

ours-6-new: i think it 's important to note that a lot of the " liberal " news outlets are reporting off the top of the news . it 's true that there are a lot of people out there who do n't agree with them , but it 's hard to argue that it 's fair to assume that all news outlets are going to be able to see the news they 're talking about . it 's not fair to say that fox news does n't exist , but that does n't mean it 's true . it 's just that it 's not the news , it 's the news . the news is n't going to be biased , it 's that it 's reporting on the news and reporting the news . if the news was n't going to report on the news media , it would n't be enough to cover it . it would be much easier to find a way to get news coverage .

passage-1: i use http://www.goldalert.com to check the spot gold price . i would definietly recommend gold investment to gain better leverage within the market . author profile james pethokoukis is the money & politics columnist for reuters breakingviews . previously , he was the business editor and economics columnist for u.s. news & world report . pethokoukis has written for many publications including the new york times , the weekly standard , commentary , usa today , and investor 's business daily . pethokoukis is also an official cnbc contributor . in addition , he has appeared numerous times on msnbc , fox news channel , fox business network , the mclaughlin group , cnn , and nightly business report on pbs.author profile james pethokoukis is the money & politics columnist for reuters breakingviews . previously , he was the business editor and economics columnist for u.s. news & world report . pethokoukis has written for many publications including the new york times , the weekly standard , commentary , usa today , and investor 's business daily . pethokoukis is also an official cnbc contributor . in addition , he has appeared numerous times on msnbc , fox news channel , fox business network , the mclaughlin group , cnn , and nightly business report on pbs . a graduate of northwestern university and the medill school of journalism , pethokoukis is a 2002 jeopardy! champion . james.pethokoukis@thomsonreuters.com


passage-2: cnn is the only remaining cable news network to do everything close to right when it comes to covering the news . fox news and msnbc are ahead because people like sensation . o’reilly is number one because of his opinions . his show in itself is fine . but fox news programs , that are supposed to be neutral , are biased to say the least . fair and balanced , fox is not . on the same token , msnbc is the same than fox , just on the liberal side . cnn appears to be in the middle and sort of does good work . of course , no-one is watching because there is no controversy when they do their work .

passage-3: if fox news was not on the air it you would get the impression that everything liberal politicians do is dandy and everything republicans do is to protect the rich . if fox is only weakly countered by msnbc ( and cnn ) it is because the network news watching audience tends to favor a conservative viewpoint , not because the converage itself is any less biased . [ ... ] tweet check out this interesting story : the fox in the tea party – reuters blogs [ ... ] posted by the fox in the tea party &#8211; reuters blogs &#8211; san francisco luxury living | san francisco luxury living | report as abusive dec 22 , 2011 2:36 am utc fox news viewers are also consistently the most poorly informed regarding the facts of current events 
--------------------------------------------------------------------
CMV: It should be Illegal to smoke in public, even outdoors.

ours-6-new: i do n't want to live in a world where i live in a country where smoking is illegal , but i do n't think it 's safe to say that smoking should be illegal . i do n't see any reason why it should n't be illegal . it 's not illegal to smoke in public , it 's just a matter of public policy . it 's a matter of law enforcement , and it 's illegal to have a place in place to make sure that the public is n't going to do anything about it . it 's the government 's job to make sure the public wants to keep it safe . it 's

passage-1: in northern ireland , a smoke-free law has been in effect since 30 april 2007 . it is illegal to smoke in all enclosed workplaces . this includes bars , restaurants , offices ( even if the smoker is the only person in the office ) and public buildings . like scotland , the smoke-free law is comprehensive in that places such as telephone boxes and enclosed bus/train shelters are included . the on-the-spot fine for smoking in a workplace is £ 50 ( ~ € 70 / ~ \$ 100 ) , while a business that allows smoking can be fined £ 2,500 ( ~ € 3,700 / ~ \$ 5,000 ) .

passage-2: i worry about the example that it sets for people ( read : children ) who will look to him as a role model . he seems like a pretty upstanding person in general , heck , i idolize the guy a bit and i ’m not a kid . for all of his good qualities , what message will his smoking send to impressionable young minds ? if he does take it up again , or if he is smoking now , i hope that it is n’t publicized a bunch and that he is n’t overt about it . i feel the same way about celebrities and other politicians too though ! geez . barack obama has obviously benefited enormously from kicking his smoking habit ; he ’s lucky to have that kind of support from his very smart wife .


passage-3: " would it be alright for the government to ban smoking in all public places ? " it depends on what you mean by " public . " i would say yes , if you mean truly public places like government buildings . the public essentially owns those buildings and smoking can , and probably should , be banned there . if , however , by " public " you mean any place that people gather , like restaurants or bars , then no . these are private businesses . their smoking policies should be determined by the owners and customers . if people do n't like their policies , then people can go somewhere else . " or do the rights of smokers to light up in public trump my rights to breathe smoke-free air ? "

--------------------------------------------------------------------
CMV: Making the minimum wage a “living wage” is an impractical goal

ours-6-new: it 's not the government 's job to set the minimum wage , it 's to make sure that everyone has the right to do whatever they want . if you do n't want to live in a world where it 's a living wage , you 're going to be able to find a living wage where you ca n't afford to pay for it . you ca n't force you to pay for your labor if you ca n't work . if you have a job , you have to pay enough to do so . if you 're working at a factory , you 're not going to have to worry about it . you do n't need
 
passage-1: a state administrative board appointed by mr. cuomo also set a \$ 15 hourly wage for fast-food workers last summer . “ raising the minimum wage empowers workers with a fair salary , helps them support their families with dignity , and grows the economy for all , ” mr. cuomo said in a statement . “ the staff at nebraskaland joins fast-food workers as well as state and suny employees who experience the transformative impact of a living wage , and i commend the company for leading by example . ” image nebraskaland , which decided last year to begin raising its minimum wage to \$ 15 from \$ 10 an hour , expects to spend an additional \$ 350,000 annually on salaries.creditángel franco/the new york times supporters of the increase , including leaders in the democratically controlled assembly and labor unions , say that it would benefit workers and local economies .

passage-2: the fair labor standards act establishes a minimum wage at the federal level that all states must abide by , among other provisions . fourteen states and a number of cities have set their own minimum wage rates that are higher than the federal level . for certain federal or state government contacts , employers must pay the so-called prevailing wage as determined according to the davis-bacon act or its state equivalent . activists have undertaken to promote the idea of a living wage rate which account for living expenses and other basic necessities , setting the living wage rate much higher than current minimum wage laws require.for certain federal or state government contacts , employers must pay the so-called prevailing wage as determined according to the davis-bacon act or its state equivalent . activists have undertaken to promote the idea of a living wage rate which account for living expenses and other basic necessities , setting the living wage rate much higher than current minimum wage laws require . the minimum wage rate is there to protect the well being of the working class .

passage-3: the code says a factory must pay at least the minimum wage of the country where it is situated , with an eye to tying wages to the workers ' basic needs . the compromise on wages was adopted after labor and human rights members demanded wages that would support a family , while apparel companies said they should only have to pay the minimum wage . both sides expect arguments over wage levels in countries like haiti and indonesia , where the minimum wage is too low to support a family . '' unless we talk about a living wage and start to define it , a sweatshop will always be a sweatshop , '' said medea benjamin , who heads global exchange , a human rights group not on the task force .
 
 
 
--------------------------------------------------------------------
CMV: employers should be allowed to discriminate against pregnant women

ours-6-new: i think it 's important to note that a woman 's right to bodily autonomy is an important part of her job , and that she should be able to refuse to work with her employer if she does n't want to . i do n't think it 's fair to say that she should have the right to refuse service to her employer , but that does n't mean she should n't be allowed to do so . i 'm not saying she should be forced to do that , but i do n't believe she should be allowed to refuse to serve her because of her lack of respect for her partner . i think that it 's not fair to say she should n't have to pay for it , but i think it should also be noted that the risk is too much of a commitment to her . it 's about her right to not be able to do anything about it . it does n't matter if the

passage-1: if an employee is temporarily unable to perform her job due to pregnancy , the employer must treat her the same as any other temporarily disabled employee ; for example , by providing light duty , modified tasks , alternative assignments , disability leave , or leave without pay . an employer may have to provide a reasonable accommodation for a disability related to pregnancy , absent undue hardship ( significant difficulty or expense ) . "

passage-2: these general job duties are not all inclusive and team members will be required to undertake additional duties and responsibilities as may be necessary to service customer needs . toys ' r'us is an equal-opportunity employer and is committed to providing a workplace free from harassment or discrimination . all employment decisions are to be made without regard to race , color , age , gender , sexual orientation , religion , marital status , pregnancy , national origin/ancestry , citizenship , physical/mental disability , military status or any other basis prohibited . toys ' r'us is an equal-opportunity employer and is committed to providing a workplace free from harassment or discrimination . all employment decisions are to be made without regard to race , color , age , gender , sexual orientation , religion , marital status , pregnancy , national origin/ancestry , citizenship , physical/mental disability , military status or any other basis prohibited by law .

passage-3: the agency said that an employer may not treat pregnant workers differently from employees who are similar in their ability or inability to work based on the cause of their limitations . it said employers must provide light duty to pregnant workers on the same terms that light duty is offered to employees injured on the job who have a similar work limitation . moreover , the commission said that an employer may not force an employee to take a leave because she is or has been pregnant , as long as she is able to perform her job . for an employer to require a worker to take a leave would violate the pregnancy discrimination act even if the employer believes it is acting in the employee ’s best interest.moreover , the commission said that an employer may not force an employee to take a leave because she is or has been pregnant , as long as she is able to perform her job . for an employer to require a worker to take a leave would violate the pregnancy discrimination act even if the employer believes it is acting in the employee ’s best interest . employers that offer health insurance plans , the commission said , must apply the same terms and conditions to pregnancy-related costs as it does to medical costs unrelated to pregnancy .

--------------------------------------------------------------------
CMV: America should legalize all drugs.

ours-6-new: drug use is one of the most addictive drugs in the world . if you want to get rid of drugs , you 're going to need to have a hard time getting rid of drugs . if you do n't want to do drugs , you need to be able to keep yourself safe . you ca n't just go to jail if you 're not going to go to jail for drug use . if you 're a drug addict , you should n't have to deal with it . if you are going to jail for it , you have to make sure that you are n't going to do it again . you do n't have to worry about getting caught , you 're just going to have to go to the store and get a job . you have to wait until you can get away with it . it 's not like it 's just a matter of how much money you have to spend on drugs .

passage-1: why do people use illegal drugs ? mary o'grady 's " drug gangs have mexico on the ropes " ( americas , jan. 26 ) is very interesting because she has correctly identified our demand for drugs as a major contributor to this serious threat . legalizing drugs to remove the price premium would indeed lower the drug gang income , but the dutch experience with legalizing drugs shows that such a policy would only alleviate some social problems for a little while . in addition , it is simply wrong for a government to encourage people to fall into the insatiable craving of a drug addiction . why do so many people in the u.s. buy illegal drugs ?

passage-2: legalize all drugs . it would shut the cartels down almost immediately . and it ’s not like the drugs are n’t already here . ask any police officer or dea man . mexican drugs can be bought anywhere in america right now . education , clinics to help the drug users and strict drug testing by employers will shut the drugs down . particularly when there is no longer a lucrative drug market for the criminals . more than half the people in this country are incarcerated because of drugs . making drugs illegal is causing substantially more damage than legalization ever will . prohibition did n’t work either . make drugs legal , tax them and shut down the criminal enterprises .

passage-3: the cops would go hog wild arresting hard drug users to get them into the prisons till there is none left to influence new users . . marijuana needs to be legalized though . . there is n’t even close to enough prison space for all of that , and it is harmless anyways . just hard drug users … the government could purchase or contract the drugs from the producers in columbia , afganistan , etc and cut out the criminals from the profits . . eliminating street gangs and drug cartels . . afghanistan will sell pharmaceutical grade morphine and float the company on the us stock exchange . with permits issued by the government to allow the poppy to be grown .



